Action Detection from a Robot-Car Perspective

We present the new Road Event and Activity Detection (READ) dataset, designed and created from an autonomous vehicle perspective to take action detection challenges to autonomous driving. READ will give scholars in computer vision, smart cars and machine learning at large the opportunity to conduct research into exciting new problems such as understanding complex (road) activities, discerning the behaviour of sentient agents, and predicting both the label and the location of future actions and events, with the final goal of supporting autonomous decision making.

==> text/contrib.tex <==
\\
\noindent 
\textbf{Contributions:}
We contribute a dataset which
\begin{itemize}
\item can be used for action detection from car's perspective
\item it can be used for to anticipate the future action labels and future locations of current actions
\end{itemize}

==> text/tramnet_approach.tex <==
% deep recofigurable feature pooling for action detection
\section{Methodology}~\label{sec:methodology}
\begin{figure*}[t]
  \centering
  \includegraphics[scale=0.19]{figures/methodology/base_net.pdf}
  \vspace{-0.2cm}
  \caption{
    {\small
      \textit{Base network architecture.
      \textbf{(a)} SSD convolutional layers;
      \textbf{(b)} the corresponding conv feature maps outputted by each conv layer;
      \textbf{(c)} $r$ anchor boxes with different aspect ratios
      assigned to cell location $c_5$ of the $3 \times 3$ feature map grid;
      \textbf{(d)} transition matrices for the $P$ feature map grids in the pyramid, where $P=6$.
      }
    }
 }
\label{fig:base_net}
\vspace{-0.7cm}
\end{figure*}
%----------------------------------------------------------------------------
% \vspace{-0.2cm}
In Section~\ref{subsec:base_network},
we introduce the base network architecture used for feature learning.
We cast the action proposal generation problem
in a hidden Markov model (HMM) formulation (\S~Section~\ref{subsec:hmm}),
and introduce an approximate estimation
of the HMM transition probability matrix using
a heuristic approach (\S~Section~\ref{subsec:transition_matrix}).
% ( Section~\ref{subsec:hmm}),
The proposed approximation is relatively inexpensive
and works gracefully (\S~\ref{subsec:discussion}). % TODO refer experiments with trans matrix
%----------------------------------------------------------------------------
In Section~\ref{subsec:reconfig_pooling_layer},
a configurable pooling layer architecture is presented
which pools convolutional features from the regions in the two frames linked by the estimated transition probabilities.
%----------------------------------------------------------------------------
Finally, the output layers of the network (i.e., the micro-tube
regression and classification layers) are described in Section~\ref{subsec:conv_2_linear}.

% in the base network tell that this is SSD based,
% draw a diagram for the add conv layers and the 6 feature maps
% then show the anchor for only one cell location in the 5x5 grid

\subsection{Base network} \label{subsec:base_network}
The base network takes as inputs a pair of video frames
$(f_t,f_{t+\Delta})$ and propagates them through two parallel CNN streams
(cf. Fig.~\ref{fig:algorithmOverview}~\textbf{(b)}).
In Fig.~\ref{fig:base_net}~\textbf{(a)},
we show the network diagram of one of the CNN streams; the other follows the same design.
\\
The network architecture is based on Single-Shot-Detector (SSD)~\cite{liu15ssd}.
The CNN stream outputs a set of $P$ convolutional feature maps
$K_{p}$, $p = \{ 1,2, ..., P = 6 \}$
(feature pyramid, cfr. Fig.~\ref{fig:base_net}~\textbf{(b)})
of shape $[H'_{p} \times W'_{p} \times D_p]$,
where $H'_{p}$, $W'_{p}$ and $D_p$ are the height, width and depth
of the feature map at network depth $p$, respectively.
%Indeed the feature maps are extracted at different depths $p = \{ 1,2, ..., 6 \}$ of the network.
For $P=6$ %different network depth levels,
the conv feature map spatial dimensions are $H' = W' = \{ 38, 19, 10, 5, 3, 1\}$, respectively.
The feature maps at the lower depth levels (i.e., $p=1,2$ or 3)
are responsible for encoding smaller objects/actions,
whereas feature maps at higher depth levels encode
larger actions/objects.
For each cell location $c_{ij}$ of $[H'_{p} \times W'_{p}]$ feature map grid $\mathbf{C_p}$,
$r$ anchor boxes (with different aspect ratios)
are assigned where $r_{p} = \{ 4, 6, 6, 6, 4, 4 \}$.
E.g.
% at network depth $p=5$,
% we extract a conv feature map of shpae $[3 \times 3 \times 256]$,
at each cell location of the $3 \times 3$ grid in the pyramid,
$4$ anchor boxes are produced
(Fig.~\ref{fig:base_net}~\textbf{(c)}),
resulting in a total of $3 \times 3  \times 4 = 36$ anchor boxes.
These anchor boxes, assigned for all $P=6$ distinct feature map grids,
are then used to generate action proposal hypotheses based on the
transition probability matrix, as explained below.

Note that the proposed framework is not limited to any particular base network architecture,
and is flexible enough to accommodate any latest network~\cite{lin2017focal,carreira2017quo}. 
% with greater representation power.

\subsection{HMM-based action proposal generation} \label{subsec:hmm}
A \emph{hidden Markov model} (HMM) models a time series of (directly measurable) \emph{observations} $\mathbf{O} = \{ \mathbf{o}_1, \mathbf{o}_2, ..., \mathbf{o}_T\}$, either discrete or continuous, as randomly generated at each time instant $t$ by a \emph{hidden state} $\mathbf{q}_t \in \mathbf{Q} = \{ \mathbf{q}_1, \mathbf{q}_2, ..., \mathbf{q}_{N} \}$, whose series form a Markov chain, i.e., the conditional probability of the state at time $t$ given $\mathbf{q}_1,...,\mathbf{q}_{t-1}$ only depends on the value of the state $\mathbf{q}_{t-1}$ at time $t-1$. The whole information on the time series' dynamics is thus contained in a \emph{transition probability matrix}
$\mathbf{A} = [p_{ij}; i,j=1,..,n]$,
where $p_{ij} = P(\mathbf{q}_j|\mathbf{q}_i)$ is the probability of moving from state $i$ to state $j$, and $\sum^{N}_{j=1} p_{ij} = 1$ $\forall i$.
\\
In our setting, a state $\mathbf{q}_n$ is a vector containing the 2D bounding-box coordinates
of one of the anchor boxes
$[x^{a}_{min}, y^{a}_{min}, x^{a}_{max}, y^{a}_{max}]'$ %Fabio: why the superscript ``a''?
in one of the grids forming the pyramid (\S~\ref{subsec:base_network}).
The transition matrix encodes the probabilities of a temporal link existing between
an anchor box (indexed by $i$) at time $t$ and another anchor box (indexed by $j$) at time $t+\Delta$. The continuous observations $\mathbf{o}_t$, $t=1,...,T$ are the ground-truth bounding boxes, so that $\mathbf{O}$ corresponds to a ground-truth action tube.

In hidden Markov models, observations are assumed to be Gaussian distributed given a state $\mathbf{q}_i$, with mean $\mathbf{o}_\mu^i$ and covariance $\mathbf{Q}_\Sigma^i$.
After assuming an appropriate distribution for the initial state, e.g. $P(\mathbf{q}_0)\sim \mathcal{N}(0,I)$, the transition model $A = [P(\mathbf{q}_j|\mathbf{q}_i)]$ allows us to predict at each time $t$ the probability $P(\mathbf{q}_t | \mathbf{O}_{1:t})$ of the current state given the history of previous observations, i.e.,
the probability of each anchor box at time $t$ given the observed (partial)
ground-truth action tube.
Given a training set, the optimal HMM parameters ($A$, $\mathbf{o}_\mu^i$ and $\mathbf{Q}_\Sigma^i$ for $i=1,...,N$) can be learned using standard expectation maximisation (EM) or the Baum-Welch algorithm, by optimising the likelihood of the predictions $P(\mathbf{q}_t | \mathbf{O}_{1:t})$ produced by the model.
\\
%TODO: Fabio please look at these three paragraphs see if we save space - OK
Once training is done, at test time,
the mean
$\mathbf{o}_\mu^{\hat{\mathbf{q}}_t}$ of the conditional distribution of the observations given the state associated with the predicted state $\hat{\mathbf{q}}_t \doteq \arg \max_i P(\mathbf{q}_i|\mathbf{O}_{1:t})$ at time $t$
%of the learnt state distribution $\mathbf{Q}_{\mu}$
can be used to initialise the anchor boxes for each of the $P$ CNN feature map grids (\S~\ref{subsec:base_network}).
% for a training pair $(f_t,f_{t+\Delta})$
The learnt transition matrix $\mathbf{A}$ can be used to
generate a set of training action proposals hypotheses (i.e., anchor micro-tubes, Fig.~\ref{fig:opt_prop}).
As in our case the mean vectors $\mathbf{o}_\mu^i$, $i=1,..., N$ are known a-priori
(as the coordinates of the anchor boxes are predefined
for each feature map grid, \S~\ref{subsec:base_network}),
%we initialise the mean of the hidden state  $\mathbf{Q}_{\mu}$ with the anchor box coordinates
we do not allow the M-step of EM algorithm to update $\mathbf{Q}_{\mu} = [\mathbf{o}_\mu^i, i=1,...,N]$. Only the covariance matrix $\mathbf{Q}_{\Sigma}$ is updated.
% update the $Q_{\mu}$ at m-step of EM algorithm,

\subsection{\textbf{Approximation of the HMM transition matrix}}  \label{subsec:transition_matrix}

Although the above setting perfectly formalises the anchor box-ground truth detection relation over the time series of training frames,
a number of computational issues arise. At training time,
some states (anchor boxes)
may not be associated with any of the observations (ground-truth boxes) in the E-step, leading to
zero covariance for those states. % resulting in a non-positive definite covariance matrix.
%In addition, we observe during the HMM training that
Furthermore, for a large number of states (in our case $N = 8732$ anchor boxes),
it takes around $4$ days to complete a single HMM training iteration.
\\
%In response, we propose an approximation of HMM learning based on a heuristic approach.
In response, we propose to approximate the HMM's transition probability matrix $\mathbf{A}$ with
a matrix $\mathbf{\hat{A}}$ generated by a heuristic approach explained below.

The problem is to learn a transition probability, i.e.,
the probability of a temporal link (edge)
between two anchor boxes $\{b^{a}_{t}, b^{a}_{t+\Delta}\}$
belonging to two feature map grids
$\mathbf{C}^{t}_{p}$ and $\mathbf{C}^{t+\Delta}_{p'}$.
%There are $p$ such pairs of grids corresponding to $p$ feature maps outputted by the base network (\S~\ref{subsec:base_network} Fig.~\ref{fig:base_net}~\textbf{(b)}).
If we assume that transitions only take place between states at the same level $p = p'$ of the feature pyramid, the two sets of anchor boxes
$\mathcal{B}^{t}_{p} = \{ b^{a}_{t_{1}}, ..., b^{a}_{t_{N}} \}$ and
$\mathcal{B}^{t+\Delta}_{p} = \{b^{a}_{{(t+\Delta)}_{1}}, ..., b^{a}_{{(t+\Delta)}_{N}}\}$
belonging to a pair of grids
$\{\mathbf{C}^{t}_{p},\mathbf{C}^{t+\Delta}_{p}\}$
are identical, namely:
$\mathcal{B}^{t}_{p} = \mathcal{B}^{t+\Delta}_{p} \doteq \mathcal{B}_{p} = \{b^a_i, i=1,...,N\}$,
allowing us to remove the time superscript. % $t$ and $t+\Delta$ and represent the set of all anchor boxes as $\mathcal{B}_{p}$ for clarity.
Recall that each feature map grid $C_{p}$ has spatial dimension $[H'_{p} \times W'_{p}]$.
\\
We compute a transition probability matrix $\mathbf{\hat{A}}_{p}$ \emph{individually for each grid level} $p$, resulting in $p$ such matrices of shape $[(H'_{p})^2 \times (W'_{p})^2]$ (see Fig.~\ref{fig:base_net}~\textbf{(d)}).
For example, at level $p=5$ we have a $3 \times 3$ feature map grids, so that
the transition matrix $\mathbf{\hat{A}}_{p}$ will be $[3^2 \times 3^2]$.
Each cell in the grid is assigned to $r_{p}$ anchor boxes, resulting in
$n = H'_{p} \times W'_{p} \times r_{p}$ total anchor boxes per grid
(\S~\ref{subsec:base_network}).
%Note that here we are interested in learning a transition probability between
%two anchor boxes %$b^{a}_{loc_{1}}$ and $b^{a}_{loc_{2}}$
%belonging to two different cell locations
%%%%%$c_{loc_{1}}$, $c_{loc_{2}}$
%in the grid, % where $loc_{1} \neq loc_{2}$ thus,
%thus further reducing the search space complexity from
%$\mathcal{O}(n^f)$ to $\mathcal{O}(L^f)$
%where, $L$ is the number of cell locations in a grid.
\vspace{-0.25cm}
\paragraph{\textbf{Transition matrix computation.}}
Initially, all entries of the transition matrix are set to zero:
$\mathbf{\hat{A}}[i,j] = 0$.
Given a ground-truth micro-tube $\mathbf{m}^{g} = \{b^{g}_{t}, b^{g}_{t+\Delta}\}$
(a pair of temporally linked ground-truth boxes~\cite{saha2017amtnet}),
%belonging to the training set,
we compute the IoU overlap for each ground-truth box
with all the anchor boxes $\mathcal{B}_{p}$ in the considered grid, namely:
$IoU(b^{g}_{t}, \mathcal{B}_{p})$ and $IoU(b^{g}_{t+\Delta}, \mathcal{B}_{p})$.
We select the pair of anchor boxes
%$\mathbf{m}^{a} = \{ b^{a}_{loc_{1}}, b^{a}_{loc_{2}} \}$
$\mathbf{m}^{a} = \{ b^{a}_{i}, b^{a}_{j} \}$
(which we term \emph{anchor micro-tube})
having the maximum IoU overlap with $\mathbf{m}^{g}$,
where $i$ and $j$ are two cell locations.
If $i = j$ (the resulting anchor boxes are in the same location) we get an anchor cuboid, otherwise a general anchor micro-tube.
\\
%%and we only consider pairs if $loc_{1} \neq loc_{2}$ i.e. $i \neq j$.
This is repeated for all $P$ feature map grids $\mathbf{C}_{p}$
to select the anchor micro-tube $\mathbf{m}^{a}_{p}$ with the highest overlap.
The best match anchor micro-tube $\mathbf{m}^{a}_{\hat{p}}$
for a given ground-truth micro-tube $\mathbf{m}^{g}$
is selected among those $P$, and
%and we vote for the corresponding cells (anchor regions) $i$ and $j$ by updating 
the transition matrix is updated as follows:
%$\mathbf{\hat{A}}[loc_{1}, loc_{2}] = \mathbf{\hat{A}}[loc_{1}, loc_{2}] + 1$.
$\mathbf{\hat{A}}[i, j] = \mathbf{\hat{A}}[i, j] + 1$.
The above steps are repeated for all the ground-truth micro-tubes in a training set.
Finally, each row of the transition matrix $\mathbf{\hat{A}}$ is normalised by dividing
each entry by the sum of that row.
\\
Fig.~\ref{fig:trans_mat} plots the transition matrix $\mathbf{\hat{A}}_p$ for $p=4$ (a feature map grid $5 \times 5$), for different values of $\Delta$.
As explained in the following, the configurable pooling layer
employs these matrices to pool conv features for action proposal classification and regression.

Although our approach learns transition probabilities for anchor boxes
belonging to the same feature map grid $\mathbf{C}_{p}$, we realise that
the quality of the resulting action proposals could be further
improved by learning transitions between anchors
across different levels of the pyramid. %$\mathbf{C}_{p}$s. 
As the feature dimension of each map varies in SSD, e.g. 1024 for $p=2$ and 512 for $p=1$, a more consistent network such as FPN~\cite{lin2017focal} with Resnet~\cite{he2016deep} would be a better choice as base architecture. Here we stick to SSD to produce a fair comparison with~\cite{kalogeiton2017action,singh2016online,saha2017amtnet}, and
leave this extension to future work.


\begin{figure*}[h]
  \vspace{-0.4cm}
  \centering
  \includegraphics[scale=0.16]{figures/methodology/transmat_mcsampl.pdf}
   \vskip -0.4cm
  \caption{
    {\small
      \textit{
      \textbf{(a)}
      Transition matrix for a $5 \times 5$ feature map grid ($p=4$)
      for different $\Delta$ values.
      As $\Delta$ increases,
      off-diagonal probability values also increase,
      indicating a need for anchor micro-tubes rather than anchor-cuboids.
      \textbf{(b)} {Top - Monte Carlo sampling of transition hypotheses $(i,j) \in \mathbf{C}_{p} \times \mathbf{C}_{p}$ based on uniformly sampling the $[0,1]$ range. Bottom - our anchor micro-tube sampling scheme, based on thresholding the transition probabilities $p(i|j)$, is also stochastic in nature and emulates Monte Carlo sampling. The blue line denotes the threshold and the shaded area above the threshold line shows the sampling region, a subset of the product grid $\mathbf{C}_{p} \times \mathbf{C}_{p}$.}
      }
    }
 }
\label{fig:trans_mat}
\vspace{-7mm}
\end{figure*}


\subsection{Configurable pooling layer} \label{subsec:reconfig_pooling_layer}
The SSD~\cite{liu15ssd} network uses convolutional kernels of dimension
$[3 \times 3 \times D]$ as classification and regression layers (called \emph{classification} and \emph{regression heads}).
More specifically, SSD uses $r \times 4$ kernels for bounding box regression
(recall $r$ anchor boxes with different aspect ratios are assigned to each cell location (\S~\ref{subsec:base_network}))
and $(C+1) \times r$ kernels for classification over the $p$ conv feature maps
(\S~\ref{subsec:base_network}). This is fine when the number of proposal hypotheses
is fixed (e.g., for object detection in images, the number of anchor boxes is set to $8732$).
In our setting, however,
the number of proposals varies depending upon the cardinality of transition matrix
$| \mathbf{\hat{A}}_{p} |$ (\S~\ref{subsec:transition_matrix}).
Consequently, it is more principled to implement the classification and regression heads
as fully connected layers (see Fig.~\ref{fig:algorithmOverview}~\textbf{(f)}).
%In case of lot of consistent (for eg. all cell only move to one step in either direction)
% \SAHA{Suman: not clear:-}
If we observe consistent off-diagonal entries in the transition matrices (e.g. lots of cells moving one step in the same direction),
we could perform pooling as convolution feature map stacking with padding to allow spatial movement.
% in the feature maps.
However, transition matrices are empirically extremely sparse 
(e.g., there are only 25 and 1908 off-diagonal non-zero entries in the transition matrices at $\Delta$ equal to 4 and 20, respectively, on the UCF101-24 dataset).

% Fabio: we should probably expand on this to address the ECCV reviewer criticism
\textbf{Anchor micro-tube sampling.}
% In addition, 
Each transition matrix is converted into a binary one by thresholding, so that the cardinality of the matrix depends not only on the data but also on the transition probability threshold. 
{Our transition matrix based anchor micro-tube sampling scheme is stochastic in nature and emulates Monte Carlo sampling technique (Fig.~\ref{fig:trans_mat} (b)). 
A thresholding on the transition matrix allows us to sample a variable number of anchors rather than a fixed one.}  
We empirically found that a 10\% threshold gives the best results in all of our tests. We discuss the threshold and its effect on performance in \S~\ref{subsec:transition_matrix}. 

The pooling layer (see Fig.~\ref{fig:algorithmOverview}~\textbf{(d)}) is configured to
pool features from a pair of convolutional feature maps
$\{K^{t}_{p}$, $K^{t+\Delta}_{p}\}$ each of shape
$[H'_{p} \times W'_{p} \times D]$.
The pooling is done at cell locations %$loc_1$ and $loc_2$ for feature maps $K^{t}_{p}$ and $K^{t+\Delta}_{p}$
$i$ and $j$,
%respectively, where the cell locations are defined
specified by the estimated (thresholded) transition matrix $\mathbf{\hat{A}}_p$ (\S~\ref{subsec:transition_matrix}).
The pooling kernel has dimension $[3 \times 3 \times D]$.
Pooled features are subsequently stacked
(Fig.~\ref{fig:algorithmOverview}~\textbf{(e)})
to get a single feature representation of a shape
$[2 \times 3 \times 3 \times D]$ per anchor micro-tube.
\iffalse
\textbf{Generality at Test Time.} 
Our approach allows the pooling layer to be \emph{``configurable''}
for a specific set of transition matrices,
while keeping the number of network parameters intact
by simply replacing the convolution heads with linear layers.
Another big advantage of using a transition matrix
% based reconfigurable pooling layer
is that, at test time, we can generate a more generic set of anchor micro-tubes
by setting the transition probabilities to $1$ for those off-diagonal entries
which were earlier $0$ for the training set, or accommodating all anchor micro-tubes transitions relative to each cell.
At test time, in cases in which test $\Delta$ is larger than 1, 
we use linear interpolation to generate the missing detection boxes within a micro-tube.
\fi
\subsection{Classification and regression layers} \label{subsec:conv_2_linear}
%\red{[Note for Gurkirt: please check this section.]}\\
After pooling and stacking, we get $M$ conv features of size
$[2 \times 3 \times 3 \times D]$, for each $M$ anchor micro-tube cell regions
where $M = \sum_{p=1}^{P=6} |\mathbf{\hat{A}}_p|$
is the sum of the cardinalities of the $P$ transition matrices.
We pass these $M$ features to a classification layer
$( (18 \times D)$, $((C+1) \times r) )$,
and a regression layer
$( (18 \times D)$, $((2 \times 4) \times r) )$
(see Fig.~\ref{fig:algorithmOverview}~\textbf{(f)}).
The classification layer outputs $C+1$ class scores
and the regression layer outputs $2 \times 4$ bounding-box coordinates
for $r$ anchor micro-tubes per anchor micro-tube cell region
(see Fig.~\ref{fig:algorithmOverview}~\textbf{(g)}).
The linear classification and regression layers have the
same number of parameters as the convolutional heads in the SSD network~\cite{liu15ssd}.

\subsection{Online action tube generation and temporal trimming}\label{subsub:algo}
The output of the proposed network is a set of detection micro-tubes
and their class confidence scores (see Fig.~\ref{fig:algorithmOverview}~\textbf{(g)}).
We adapt the online action tube generation algorithm
proposed by Singh~\etal~\cite{singh2016online}
to compose these detection micro-tubes into complete action paths (tracklets)
spanning the entire video.
Note that, Singh~\etal~\cite{singh2016online} use their tube generation
algorithm to temporally connect frame-level detection bounding-boxes,
whereas our modified version of the algorithm connects video-level detection
micro-tubes. Similarly to~\cite{singh2016online},
we build action paths incrementally by connecting micro-tubes across time.
as the action paths are extracted,
their temporal trimming %(to solve for temporal detection)
is performed using dynamic programming~\cite{Saha2016,Evangel-2014}.
In Section~\ref{subsec:discussion} we show that
temporal segmentation helps improve
detection performance for datasets
containing highly temporally untrimmed videos
e.g., DALY~\cite{daly2016weinzaepfel},
where on average only $4$\% of the video duration is covered by action instances.
\\
\textbf{Fusion of appearance and flow cues}
We follow a late fusion strategy~\cite{kalogeiton2017action,singh2016online}
to fuse appearance and optical flow cues, performed at test time after all the detections
are extracted from the two streams.
Kalogeiton~\etal~\cite{kalogeiton2017action}
demonstrated that
\textit{mean} fusion works better than both 
\textit{boost} fusion~\cite{Saha2016} and
\textit{union-set} fusion~\cite{singh2016online}.
Thus, in this work we produce all results (cf. Section~\ref{subsec:discussion})
using \textit{mean} fusion~\cite{kalogeiton2017action}.
We report an ablation study of the appearance and flow stream performance
in the supplementary material.
